Cogniculture: Towards a Better Human-Machine Co-evolution

Research in Artificial Intelligence is breaking technology barriers every day. New algorithms and high performance computing are making things possible which we could only have imagined earlier. Though the enhancements in AI are making life easier for human beings day by day, there is constant fear that AI based systems will pose a threat to humanity. People in AI community have diverse set of opinions regarding the pros and cons of AI mimicking human behavior. Instead of worrying about AI advancements, we propose a novel idea of cognitive agents, including both human and machines, living together in a complex adaptive ecosystem, collaborating on human computation for producing essential social goods while promoting sustenance, survival and evolution of the agents' life cycle. We highlight several research challenges and technology barriers in achieving this goal. We propose a governance mechanism around this ecosystem to ensure ethical behaviors of all cognitive agents. Along with a novel set of use-cases of Cogniculture, we discuss the road map ahead for this journey.

==> cogniculture-definition.tex <==
\subsection{Definition and analogy from other *culture definitions. [Rakesh]}
\label{sec:cogniculture-definition}

==> cogniculture-technology-differentiators.tex <==
\subsection{Key Technology Differentiators}
\label{sec:cogniculture-technology-differentiators}

\par Cognitive agents will be part of completing tasks in business context. Hence it is important for the agents to gel will with the user so that user can get the same experience while interacting with the cognitive agent as if it would have happened if it was a human agent. For this it is important for cognitive agent to evolve individually in a micro set up so that the entire muti-agent system could evolve towards betterment. Also, as agents evolve with time, it is certainly important for agents to learn to be more presentable to the user. One way to do this is to ask the user about the experience while agent completes the task and take feedback on improvement which can be then fed into underlying ML models which will make agents evolve. Also, the rating of the user could create a distinction between different agents’ skill sets and already evolved agents who are being rated highly could be promoted to more critical jobs. 
\par As it is important for agents to evolve over its time span for completing tasks, agents also need to sense, perceive, draw inferences and eventually take a decision based on its cognitive abilities. The entire procedure is needed to be operationalized through a socio-cognitive architecture which enables the agents to make reasonable decisions. 
\par In the very core of the socio-cognitive architecture it is important to have a knowledge layer which stores the inference drawn from data and this knowledge gets enriched over and over as agents gain more experience while completing tasks. In the socio-cognitive architecture knowledge layer is the most important part since the perceived knowledge is already stored in that section after sensing of the data has already been completed. Hence it is necessary to plug the knowledge layer with an AI platform which will enable agents to scrape data from different sources like blogs, news feeds, public forums etc. to understand and learn the social trends and beliefs. It is also important for cognitive watchdogs to draw knowledge from these data sources to get a demarcation between what is ethical and reasonable under the societal norm and what is not. For this reason, cognitive watch dogs are also needed to be culturally infused. The societal norms can vary from region to region, country to country and from culture to culture. Hence, it is also important for the agents as well as the watch dogs to be adaptable to multiple geographies with multiple linguistics. Through AI platform information will be collected from different sources. Some of the information could be conflicting. Also, it could happen that different data collected from different sources when summarized may lead to the same summarized knowledge. Hence it is important to have ML algorithms linked to the AI platform which enables the agents not only to make a unified set of information but also assists agents to discard conflicting information. 
\par As agents evolve over time, \Cogniculture~laws should play a key role in maintaining governance over agents' actions. For example, the cognitive watch dogs will learn the societal ethics and try to implant such ethical behaviors in agents.


current products that have some elements of culture (Rakesh can we discuss once about this....)


==> experiments-results.tex <==
\section{A Cogniculture Use-case}
\label{sec:cogniculture-use-case}
In this section, we briefly discuss a \Cogniculture~use-case that we have implemented using one of the proposed ideas of identifying cultural background of an agent in a specific application context. Many times an educational content is heavily influenced by author's own culture and may not be suitable for students coming from different cultural backgrounds. For example, an US author may give example of American Football in his content, while Indian student may relate closely with Cricket. Hence it is important for the reuse of content to culturally adapt it for target students. The use-case to identify portions of the content, which can be culturally sensitive and recommend the author possible replacement options. For 

In this solution, we extract entities from a textual content using Named Entity Recognition (NER) for every cultural aspect mentioned in subsection ``Culture is the Key". We use a corpus of 10 million Wikipedia articles to identify culture of students from their minimal demographic data that we may have. Let, $D_{X}$ be the set of Wiki articles containing a set of keywords $X$. If $A$ is an entity from content and $B$ is a set of keywords from demographic information of students, then Cultural Relevance Factor (CRF) between $A$ and $B$ is computed as 

\begingroup\makeatletter\def\f@size{7}\check@mathfonts
\begin{equation}
\textrm{CRF}_{AB} = \frac{2 \times n(D_{A} \cap D_{B}) - min\left(n(D_{A} - D_{B}),n(D_{B} - D_{A})\right)}{min\left(n(D_{A}), n(D_{B})\right)}
\end{equation}
\endgroup

$\textrm{CRF}_{AB} > 0$ indicates $A$ and $B$ are culturally relevant, hence $A$ need not be adapted. $\textrm{CRF}_{AB} < -0.85$ implies less than 5\% intersection between $D_{A}$ and $D_{B}$, hence $A$ is culturally irrelevant for target $B$ and should be adapted. $n(D_{A}) > 2000$ implies from experiments that $A$ is universal entity and need not be adapted. At last if none of above conditions are satisfied in that order, we recommend $A$ to be adapted being culturally irrelevant for target $B$.

For every $A$ recommended to be adapted, we search for Wiki articles containing $B$ and extract entities from them for every cultural aspect using NER. We find most frequent entities of cultural aspect as that of $A$ and recommend top 5 entities for replacing $A$.

Standard NER models do not support extraction of many of cultural aspect. So we trained a custom NER models for every cultural aspect using a set of 40 documents, containing about 2400 such annotations. We use three different APIs, Stanford Core NLP, Apache OpenNLP, and IBM Watson Knowledge Studio\footnote{https://www.ibm.com/us-en/marketplace/supervised-machine-learning} (IBM WKS), and tested their performance using 5 fold cross validation. Accuracy numbers are reported in table \ref{tab:ner-accuracy}. IBM WKS is observed to be performing much superior than other APIs.

\begin{center}
\begin{table}[h!]
\begin{tabular}{ |c|c|c|c| } 
\hline
\textbf{API} & \textbf{Precision} & \textbf{Recall} & \textbf{F-score} \\
\hline
IBM WKS          & 0.96 & 0.94 & 0.95  \\ 
\hline
Stanford Core NLP & 0.75 & 0.78 & 0.77 \\ 
\hline
Apache Open NLP  & 0.61 & 0.37 & 0.46  \\ 
\hline
\end{tabular}
\caption{Performance of NER APIs for extraction of cultural aspects. \label{tab:ner-accuracy}}
\end{table}
\end{center} 

If any of the top 5 recommended replacements is valid for a culturally irrelevant entity from content, we marked the recommendation as successful. In an experiment containing 215 such entities identified irrelevant for Indian students from 50 educational contents, 83\% of the times our recommendations were successful, which demonstrates the effectiveness of our approach.
